An Evaluation of Memory Optimization Methods for Training Neural Networks

As models continue to grow in size, the development of memory optimization methods (MOMs) has emerged as a solution to address the memory bottleneck encountered when training large models. To comprehensively examine the practical value of various MOMs, we have conducted a thorough analysis of existing literature from a systems perspective. Our analysis has revealed a notable challenge within the research community: the absence of standardized metrics for effectively evaluating the efficacy of MOMs. The scarcity of informative evaluation metrics hinders the ability of researchers and practitioners to compare and benchmark different approaches reliably. Consequently, drawing definitive conclusions and making informed decisions regarding the selection and application of MOMs becomes a challenging endeavor. To address the challenge, this paper summarizes the scenarios in which MOMs prove advantageous for model training. We propose the use of distinct evaluation metrics under different scenarios. By employing these metrics, we evaluate the prevailing MOMs and find that their benefits are not universal. We present insights derived from experiments and discuss the circumstances in which they can be advantageous.

==> trash/5-cost-model.tex <==
\section{Performance Modeling}
In this section, we introduce a simple but effective performance model to quantitatively model and explain the experiment results in the last section.
The performance model provides predictions of training performance by estimating training throughput and evaluating the trade-off between cost and latency. 
In the next section, we will utilize the model to empower practitioners in making well-informed decisions about the optimal MOMs for their specific requirements. 

\subsection{Batch Latency Modeling}
\begin{equation}
    L(B, K) = max(a, B * \frac{C_B}{p(K)}) + b
\end{equation}
$max$ here tries to model the hardware utilization: $a$ is a fixed time consumption when the hardware is underutilized. As the batch size $B$ increases, the GPU becomes fully utilized, resulting in a linear increase in batch latency proportional to the batch size $B$. The incremental latency cost for each batch size increment is $\frac{C_B}{p(K)}$, where $C_B$ represents the floating-point operations required by the model per batch size, and $p(K)$ denotes the effective FLOPS (floating point operations per second) provided by the hardware. Notice here $p(K)$ is dependent on the number of devices $K$, as increasing the number of devices will also increase the effective FLOPS available.
Additionally, $b$ denotes a fixed execution cost that remains constant regardless of the batch size. This execution cost typically encompasses tasks such as weight updates and framework overhead. 

\subsection{Throughput Modeling}
Throughput $T$ is defined as the batch size divided by the batch latency:
\begin{equation}
    T(B, K) = \frac{B}{L(B, K)} = \frac{B}{max(a, \frac{B * C_B}{p(K)}) + b}
\end{equation}
\begin{equation}
    T(B, K) = 
    \begin{cases}
        \frac{B}{a+b}, B \leq B_s \\
        \frac{p(K)}{C_B + \frac{b}{B}}, B > B_s
    \end{cases}
\label{eq:tpt}
\end{equation}
We introduce the concept of the saturation point, denoted as $B_s=\frac{a*p}{C_B}$. 
As observed from the formula, when the batch size is smaller than the saturation point, the throughput exhibits a linear relationship with the batch size. However, when the batch size surpasses the saturation point, further increasing the batch size leads to a continued increase in throughput, albeit with diminishing returns. In essence, the saturation point represents the batch size beyond which additional increments yield diminishing improvements in throughput. 

\textbf{Maximum Throughput Modeling} 
As can be seen from Equation~\ref{eq:tpt}, throughput is a monotonic function of batch size. Therefore, the maximum throughput is achieved with the maximum batch size:
\begin{equation}
    max(T) = T(B_{max})
\label{eq:maxtpt}
\end{equation}
In the first application scenario (\textit{Fixed hardware, larger maximum throughput}), the model ($C_B$) and hardware ($p(K)$) remain the same for a given MOM so that we can get those parameters through simple profiling. Moreover, memory consumption is a linear function of batch size, we can easily get the maximum batch size and plugin in Equation~\ref{eq:maxtpt} to get the maximum throughput. 

\subsection{Maximum Model Size Modeling}
We first introduce a model amplification factor $\gamma$, which denotes the multiplication factor of the floating point operations per batch size when the model size is increased. The throughput $T$ can be rewritten as below:
\begin{equation}
    T(B, \gamma) = \frac{B}{max(a, B * \frac{\gamma C_B}{p(K)}) + b(\gamma)}
\end{equation}
\begin{equation}
    T(B, \gamma) = 
    \begin{cases}
        \frac{B}{a+b(\gamma)}, B \leq B_s \\
        \frac{p(K)}{\gamma C_B + \frac{b(\gamma)}{B}}, B > B_s
    \end{cases}
\end{equation}
Where $B_s = \frac{a * p}{\gamma C_B}$, the saturation point shifts to a smaller number as the model gets larger. 
In the second application scenario (\textit{Fixed hardware, larger model}), the batch size ($B$) and hardware $p(K)$ remain fixed. Assuming the fixed execution cost is a linear function of the amplification factor $b(\gamma)=\gamma * b$. Through simple profiling, we can fit the relationship between batch latency and model size, therefore modeling the curve between model size and throughput.

\subsection{Cost Latency Trade-off Curve Modeling}
Likewise, the cost associated with training a single batch can be calculated as the product of the GPU price ($price$) and the number of GPUs utilized ($K$), multiplied by the batch latency ($L(B, K)$). This relationship can be expressed by the following formulation.
\begin{equation}
    Cost(B, K) = L(B, K) * K * price 
\end{equation}
where,
\begin{equation}
    L(B, K) =  \max(a, B * \frac{C_B}{K * p}) + b
\end{equation}
In the above equation, we expand $p(K) = K * p$, where $p$ is the computation capability of each GPU. When GPU is fully utilized, the cost formula simplifies to 
\begin{equation}
    Cost(B, K) = \frac{L(B, K)}{L(B, K) - b} * \frac{B * C_B}{p} * price
\label{eq:cost}
\end{equation}
In the third application scenario (\textit{Fixed training setting, better cost/time trade-off}), the batch size ($B$), hardware computation capability ($p$), and model complexity ($C_B$) remain fixed, the term $\frac{B*C_B}{p}$ becomes a constant. Consequently, the aforementioned formula mathematically represents the trade-off curve between training cost and training latency.


==> trash/6-implication.tex <==
\section{Implication}
In this section, we first list interesting conclusions derived from the performance model. Then we verify the conclusion with experiments.

\subsection{When is MOM beneficial for increasing maximum throughput?}
\begin{em}
    \begin{enumerate}
        \item MOM is beneficial when the original training is underutilized.
        \item MOM is beneficial when $\frac{\beta_{0} - \beta_{MOM}}{C_B^{MOM} - C_B^{0}} > \frac{M-\delta}{b}$.
        \item MOMs are more beneficial for larger models.
        \item MOMs are more beneficial for multi-GPU data parallel training.
    \end{enumerate}
\end{em}

\textbf{MOMs are more beneficial for larger models}. In our study, we concentrate on comparing models within the same family (e.g., different layers of Bert models, GPT models with varying numbers of encoder/decoder blocks, etc.), as models from different families are not directly comparable. As models grow larger in size, the likelihood of the original training being underutilized, i.e., running out of memory before reaching the saturation point, increases. Therefore, the application of MOM becomes more advantageous as it enables an increase in the batch size and improves hardware utilization. A detailed explanation is provided in the appendix, where we outline the complete reasoning.

To validate this implication, we conducted experiments by varying the depth and width of ResNet and GPT3 models on V100 GPUs. The results, as depicted in Figure~\ref{fig:impl}, demonstrate that when the model is shallow enough (with fewer than 280 layers for ResNet or fewer than 18 layers for GPT3) or narrow (with a hidden size smaller than 248 for ResNet or 1500 for GPT3), the application of MOMs actually slows down the training process. However, as the model becomes deeper or wider, MOMs start to accelerate the training. In the most extreme case, the original training fails to execute even with a batch size of one, emphasizing the necessity of applying MOMs to enable single-GPU training. These findings provide evidence supporting the claim that the benefits of MOMs are more pronounced with increasing model depth and width.

\textbf{MOMs are more beneficial for multi-GPU data parallel training.} The intuition behind the implication is that communication makes MOMs less expensive. Communication and synchronization across multiple devices result in a substantially higher fixed execution cost $b$. 
This cost increases with the synchronous overhead when more GPUs are utilized. Consequently, as discussed above, when both the original training and MOM fully utilize the GPU, satisfying the inequality $\frac{\beta_{0} - \beta_{MOM}}{C_B^{MOM} - C_B^{0}} > \frac{M-\delta}{b}$ becomes easier, as the right side of the inequality decreases with an increase in $b$. Furthermore, the left side remains unchanged since neither the model nor the memory optimization method is altered.

We compare the maximum throughput ratio between gradient checkpointing and the original training on Bert-Large and Swin-Large on distributed data-parallel training with 1, 2, 4, 8 V100 GPUs. As shown in Figure~\ref{fig:impl}, the ratio increases by adding more GPUs. Specifically, on Bert-Large, gradient checkpointing slows down training on a single GPU setting. However, as we increase the number of GPUs, gradient checkpointing achieves a higher maximum throughput than the original training, and can speedup the training process by 1.7× when there are 8 GPUs.



